MegaFake: A Theory-Driven Dataset of Fake News Generated by Large Language Models

Fake news significantly influences decision-making processes by misleading individuals, organizations, and even governments. Large language models (LLMs), as part of generative AI, can amplify this problem by generating highly convincing fake news at scale, posing a significant threat to online information integrity. Therefore, understanding the motivations and mechanisms behind fake news generated by LLMs is crucial for effective detection and governance. In this study, we develop the LLM-Fake Theory, a theoretical framework that integrates various social psychology theories to explain machine-generated deception. Guided by this framework, we design an innovative prompt engineering pipeline that automates fake news generation using LLMs, eliminating manual annotation needs. Utilizing this pipeline, we create a theoretically informed \underline{M}achin\underline{e}-\underline{g}ener\underline{a}ted \underline{Fake} news dataset, MegaFake, derived from FakeNewsNet. Through extensive experiments with MegaFake, we advance both theoretical understanding of human-machine deception mechanisms and practical approaches to fake news detection in the LLM era.

==> cross_test_gossipcop2megafake.tex <==
\begin{table}[!ht]
\centering
% \scriptsize
\renewcommand{\arraystretch}{1.0} % 调整行高
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule[1.2pt]
\multirow{2}{*}{Model} & \multirow{2}{*}{Accuracy} & \multicolumn{3}{c}{Legitimate} & \multicolumn{3}{c}{Fake} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
 & & Precision & Recall & F1-Score & Precision & Recall & F1-Score \\
\midrule
\multicolumn{8}{c}{LLMs} \\
\midrule
\textsc{Qwen1.5-7B\textsubscript{LoRA}} & 0.4121 & \textcolor{mygreen}{\textbf{0.5534}} & 0.4809 & 0.5123 & 0.3761 & \textcolor{mygreen}{\textbf{0.4301}} & \textcolor{mygreen}{\textbf{0.3982}} \\
\textsc{LLaMA3-8B\textsubscript{LoRA}} & \textcolor{red}{\textbf{0.4351}} & 0.5430 & 0.5209 & \textcolor{mygreen}{\textbf{0.5371}} & \textcolor{red}{\textbf{0.3802}} & 0.4103 & 0.3903 \\
\textsc{ChatGLM3-6B\textsubscript{LoRA}} & 0.3922 & \textcolor{red}{\textbf{0.5617}} & 0.2563 & 0.3451 & 0.3209 & \textcolor{red}{\textbf{0.5377}} & \textcolor{red}{\textbf{0.4531}} \\
\midrule
\multicolumn{8}{c}{Deep Learning Models} \\
\midrule
\textsc{Funnel} & 0.4012 & 0.4083 & \textcolor{mygreen}{\textbf{0.6987}} & 0.5094 & 0.0985 & 0.0497 & 0.0669 \\
\textsc{BERT-Tiny} & 0.4276 & 0.5125 & 0.5492 & 0.5238 & 0.3697 & 0.3204 & 0.3426 \\
\textsc{DeCLUTR} & 0.4214 & 0.5119 & 0.5591 & 0.5335 & \textcolor{mygreen}{\textbf{0.3792}} & 0.3296 & 0.3527 \\
\textsc{ALBERT} & 0.4175 & 0.5294 & 0.5892 & \textcolor{red}{\textbf{0.5573}} & 0.3195 & 0.2698 & 0.2923 \\
\textsc{CT-BERT} & 0.3988 & 0.4092 & \textcolor{red}{\textbf{0.7032}} & 0.5098 & 0.1197 & 0.0498 & 0.0665 \\
\textsc{RoBERTa} & \textcolor{mygreen}{\textbf{0.4296}} & 0.5196 & 0.5798 & 0.5477 & 0.3603 & 0.3098 & 0.3327 \\
\bottomrule[1.2pt]
\end{tabular}}
\caption{Cross Experiment 1: We utilize GossipCop as the training set and GossipCop-based MegaFake as the testing set. The red highlighting denotes the highest performance, while the green highlighting indicates the second-highest performance.}
\label{tab:cross_g2m}
\end{table}

==> cross_test_megafake2gossipcop.tex <==
\begin{table}[!htbp]
\centering
\renewcommand{\arraystretch}{1.0}
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule[1.2pt]
\multirow{2}{*}{Model} & \multirow{2}{*}{Accuracy} & \multicolumn{3}{c}{Legitimate} & \multicolumn{3}{c}{Fake} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
& & Precision & Recall & F1-Score & Precision & Recall & F1-Score \\
\midrule
\multicolumn{8}{c}{LLMs} \\
\midrule
\textsc{Qwen1.5-7B\textsubscript{LoRA}} & 0.4199 & \textcolor{mygreen}{\textbf{0.4361}} & 0.3842 & 0.4093 & 0.2344 & \textcolor{mygreen}{\textbf{0.3187}} & \textcolor{red}{\textbf{0.2728}} \\
\textsc{LLaMA3-8B\textsubscript{LoRA}} & 0.4367 & 0.4239 & 0.4300 & \textcolor{mygreen}{\textbf{0.4269}} & 0.2553 & 0.2447 & \textcolor{mygreen}{\textbf{0.2499}} \\
\textsc{ChatGLM3-6B\textsubscript{LoRA}} & 0.3773 & \textcolor{red}{\textbf{0.4489}} & 0.2170 & 0.2956 & 0.1640 & \textcolor{red}{\textbf{0.3791}} & 0.2260 \\
\midrule
\multicolumn{8}{c}{Deep Learning Models} \\
\midrule
\textsc{Funnel} & 0.4661 & 0.3661 & \textcolor{red}{\textbf{0.5000}} & 0.4175 & 0.1000 & 0.1000 & 0.1000 \\
\textsc{BERT-Tiny} & \textcolor{mygreen}{\textbf{0.4757}} & 0.4027 & 0.4390 & 0.4205 & 0.2700 & 0.1685 & 0.2156 \\
\textsc{DeCLUTR} & \textcolor{red}{\textbf{0.4872}} & 0.4060 & \textcolor{mygreen}{\textbf{0.4515}} & \textcolor{red}{\textbf{0.4282}} & \textcolor{red}{\textbf{0.3098}} & 0.1766 & 0.2272 \\
\textsc{ALBERT} & 0.4226 & 0.3581 & 0.4207 & 0.3883 & 0.2589 & 0.2014 & 0.2274 \\
\textsc{CT-BERT} & 0.4661 & 0.3661 & \textcolor{red}{\textbf{0.5000}} & 0.4175 & 0.1000 & 0.1000 & 0.1000 \\
\textsc{RoBERTa} & 0.4751 & 0.4007 & 0.4407 & 0.4202 & \textcolor{mygreen}{\textbf{0.2727}} & 0.1603 & 0.2021 \\
\bottomrule[1.2pt]
\end{tabular}}
\caption{Cross Experiment 1: We utilize GossipCop-based MegaFake as the training set and GossipCop as the testing set. The red highlighting denotes the highest performance, while the green highlighting indicates the second-highest performance.}
\label{tab:cross_m2g}
\end{table}


==> reference_papers.tex <==
% Lucas, J., Uchendu, A., Yamashita, M., Lee, J., Rohatgi, S., & Lee, D. (2023). Fighting fire with fire: The dual role of llms in crafting and detecting elusive disinformation. arXiv preprint arXiv:2310.15515.
% Vykopal, I., Pikuliak, M., Srba, I., Moro, R., Macko, D., & Bielikova, M. (2023). Disinformation capabilities of large language models. arXiv preprint arXiv:2311.08838.
% Wu, J., & Hooi, B. (2023). Fake News in Sheep's Clothing: Robust Fake News Detection Against LLM-Empowered Style Attacks. arXiv preprint arXiv:2310.10830.
% Chen, C., & Shu, K. (2023). Can llm-generated misinformation be detected?. arXiv preprint arXiv:2309.13788.
% Huang, Y., & Sun, L. (2023). Harnessing the power of chatgpt in fake news: An in-depth exploration in generation, detection and explanation. arXiv preprint arXiv:2310.05046.
% Jiang, B., Tan, Z., Nirmal, A., & Liu, H. (2024). Disinformation detection: An evolving challenge in the age of llms. In Proceedings of the 2024 SIAM International Conference on Data Mining (SDM) (pp. 427-435). Society for Industrial and Applied Mathematics.

 
% \begin{table*}[!htbp]
% \centering
% \caption{Literature Review: Existing literature on LLM-generated fake news detection}
% \label{tab:LLM_Disinfo_Literature}
% \renewcommand{\arraystretch}{1.5} % 调整行高
% \resizebox{1\linewidth}{!}{
% \begin{tabular}{p{0.5\linewidth}cccc} % 调整列宽
% \toprule[1.5pt]
% Citation & Theory-Driven &  Dataset Created & Dataset Scale & Data Types\\
% \midrule

% Huang, et al. \cite{huang2023survey}& \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & - & -\\

% Su et al. \cite{su2023adapting} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & - & -\\

% Hu, et al. \cite{hu2024bad}& \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} &- & -\\

% Wang, et al. \cite{wang2024explainable} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} &- & -\\

% Nan, et al. \cite{nan2024let} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} &- & -\\

% Liu et al. \cite{liu2024teller} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} &- & -\\

% Zhou et al. \cite{zhou2023synthetic} & \textcolor{red}{\ding{55}} &\textcolor{red}{\ding{55}} &- & -\\

% Wu et al. \cite{wu2023fake} & \textcolor{mygreen}{\ding{51}} & \textcolor{red}{\ding{55}} & - & -\\

% Lucas et al. \cite{lucas2023fighting} & \textcolor{red}{\ding{55}} & \textcolor{mygreen}{\ding{51}} & 27K & one fake vs. one legitimate\\

% Jiang, et al. \cite{jiang2024disinformation} & \textcolor{red}{\ding{55}} & \textcolor{mygreen}{\ding{51}} & 26K & one fake vs. one legitimate\\

% Vykopal et al. \cite{vykopal2023disinformation} & \textcolor{red}{\ding{55}} & \textcolor{mygreen}{\ding{51}} & 1.2K & one fake\\

% Chen et al. \cite{chen2023can} & \textcolor{red}{\ding{55}} & \textcolor{mygreen}{\ding{51}} & 1K &seven fake\\

% Ours. & \textcolor{mygreen}{\ding{51}} & \textcolor{mygreen}{\ding{51}} & 63,967 & four fake vs. two legitimate\\
% \bottomrule[1.5pt]
% \end{tabular}}
% \end{table*}

\begin{table*}[!htbp]
\centering
\renewcommand{\arraystretch}{1.0}
\label{tab:LLM_Disinfo_Literature}
% \renewcommand{\arraystretch}{0.9} % Adjust row height
\caption{Existing studies on machine-generated fake news detection and datasets.}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lcccc} % Adjust column width
\toprule[1.2pt]
Study & Theory-Driven & Dataset Created & Dataset Scale & Data Types\\
\midrule
Huang, et al. \citeyearpar{10.1145/3703155} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & - & -\\
Su et al. \citeyearpar{su-etal-2024-adapting} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & - & -\\
Hu, et al. \citeyearpar{hu2024bad} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & - & -\\
Wang, et al. \citeyearpar{wang2024explainable} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & - & -\\
Nan, et al. \citeyearpar{10.1145/3627673.3679519} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & - & -\\
Liu et al. \citeyearpar{liu-etal-2024-teller} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & - & -\\
Zhou et al. \citeyearpar{zhou2023synthetic} & \textcolor{red}{\ding{55}} & \textcolor{red}{\ding{55}} & - & -\\
Wu et al. \citeyearpar{10.1145/3637528.3671977} & \textcolor{mygreen}{\ding{51}} & \textcolor{red}{\ding{55}} & - & -\\
Lucas et al. \citeyearpar{lucas-etal-2023-fighting} & \textcolor{red}{\ding{55}} & \textcolor{mygreen}{\ding{51}} & $\sim$27,000 & one fake vs. one legitimate\\
Jiang, et al. \citeyearpar{jiang2024disinformation} & \textcolor{red}{\ding{55}} & \textcolor{mygreen}{\ding{51}} & $\sim$26,000 & one fake vs. one legitimate\\
Vykopal et al. \citeyearpar{vykopal-etal-2024-disinformation} & \textcolor{red}{\ding{55}} & \textcolor{mygreen}{\ding{51}} & $\sim$1,200 & one fake\\
Chen et al. \citeyearpar{chen2024llmgenerated} & \textcolor{red}{\ding{55}} & \textcolor{mygreen}{\ding{51}} & $\sim$1,000 & seven fake\\
\textbf{Ours} & \textbf{\textcolor{mygreen}{\ding{51}}} & \textbf{\textcolor{mygreen}{\ding{51}}} & \textbf{170,791} & \textbf{four fake vs. two legitimate}\\
\bottomrule[1.2pt]
\end{tabular}}
\label{tab:reference}
\end{table*}
